A Large Cross-Modal Video Retrieval Dataset with Reading Comprehension

Most existing cross-modal language-to-video retrieval (VR) research focuses on single-modal input from video, i.e., visual representation, while the text is omnipresent in human environments and frequently critical to understand video. To study how to retrieve video with both modal inputs, i.e., visual and text semantic representations, we first introduce a large-scale and cross-modal Video Retrieval dataset with text reading comprehension, TextVR, which contains 42.2k sentence queries for 10.5k videos of 8 scenario domains, i.e., Street View (indoor), Street View (outdoor), Games, Sports, Driving, Activity, TV Show, and Cooking. The proposed TextVR requires one unified cross-modal model to recognize and comprehend texts, relate them to the visual context, and decide what text semantic information is vital for the video retrieval task. Besides, we present a detailed analysis of TextVR compared to the existing datasets and design a novel multimodal video retrieval baseline for the text-based video retrieval task. The dataset analysis and extensive experiments show that our TextVR benchmark provides many new technical challenges and insights from previous datasets for the video-and-language community. The project website and GitHub repo can be found at https://sites.google.com/view/loveucvpr23/guest-track and https://github.com/callsys/TextVR, respectively.

==> table/re_lexical.tex <==
\def\x{{$\footnotesize \times$}}
\footnotesize
\setlength{\tabcolsep}{3pt}
\begin{tabular}{c|ccccc}
    % \whline	
	\multirow{2}*{\makecell[c]{Method}} &
	\multicolumn{5}{c}{Language-to-Video} \cr \cline{2-6}
     ~ & R@1$\uparrow$  & R@5$\uparrow$ & R@10$\uparrow$ & MdR$\downarrow$ & MnR$\downarrow$ \cr
     % \shline \hline
	\hline 
    Lexical matching & 1.1 & 2.7 & 4.2  & 1366 & 1270.8 \\
StarVR~(Text-only ) & 11.9 & 29.0 & 38.0 & 24.0 & 215.9 \\
     % \whline 
\end{tabular} 



==> table/table_all.tex <==
\begin{subtable}[t]{3.2in}
	\centering
	\setlength{\tabcolsep}{1.2mm}
	\small 
	\begin{tabular}{l|c|ccccc}
    % \whline
    Dataset & Input Channel & R@1  & R@5 & R@10 & MdR$\downarrow$ & MnR$\downarrow$ \\
    \hline
    \multirow{2}*{\makecell[c]{MSR-VTT}} & Vision-only & 67.7 & 56.1 & 61.5& 56.1 & 61.5 \\
     & Vision \& Text & 67.7 & 56.1 & 61.5 & 56.1 & 61.5 \\
    \hline
    
    \multirow{2}*{\makecell[c]{\textvr}} & Vision-only & 67.7 & 56.1 & 61.5  & 56.1 & 61.5\\
     & Vision \& Text & 67.7 & 56.1 & 61.5  & 56.1 & 61.5\\
    
    % \whline
    \end{tabular}
    \caption{Arbitrary-Oriented Box Matching(AOBM) for text detection task on ICDAR2015~(video frames)~\cite{karatzas2015icdar}}
	\label{table:icdar15}
	\vspace{2mm}
\end{subtable}
\quad
\begin{subtable}[t]{3.2in}
	\centering
	\setlength{\tabcolsep}{1.2mm}
	\small 
	\begin{tabular}{l|ccc}
    % \whline
    Method & ${\rm ID_{F1}}$$\uparrow$  & ${\rm MOTA}$$\uparrow$ & ${\rm MOTP}$$\uparrow$ \\
    \hline
    ours,w/o AOBM & 41.1 & 18.4 & 68.7 \\
    ours,w/ AOBM($L1$) & 63.3 & 45.6 & 76.1  \\
    ours,w/ AOBM($Cosine$) & \textbf{65.5} & \textbf{47.5} & \textbf{76.2}  \\
    
    % \whline
    \end{tabular}
    \caption{Arbitrary-Oriented Box Matching(AOBM) for text tracking task on ICDAR2015~(video)~\cite{karatzas2015icdar}.}
	\label{table:icdar15video}
	\vspace{2mm}
\end{subtable}
\quad
\begin{subtable}[t]{3.2in}
	\centering
	\setlength{\tabcolsep}{0.9mm}
	\small
	\begin{tabular}{l|ccccc}
    Length & ${\rm ID_{F1}}$$\uparrow$  & ${\rm MOTA}$$\uparrow$ & ${\rm MOTP}$$\uparrow$ & ${\rm M\mbox{-}Tracked}$$\uparrow$ & ${\rm M\mbox{-}Lost}$$\downarrow$ \\
    \hline
    % 2 & 59.2 & 42.1 & 76.2 & 36.7 & 30.2 \\
    3 & 61.2 & 44.8 & 76.1 & 38.9 & 32.6 \\
    4 & 63.4 & 45.5 & 75.9 & 40.1 & 33.2 \\
    5 & 65.2 & 47.1 & 75.9 & 42.0 & 31.5 \\
    6 & \textbf{65.5} & \textbf{47.5} & \textbf{76.2} & \textbf{43.4} & \textbf{31.3} \\
    
    % \whline
    \end{tabular}
    \caption{The input video frame length for text tracking task on ICDAR2015~(video)~\cite{karatzas2015icdar}.}
	\label{table:length}
	\vspace{2mm}
\end{subtable}
\quad
\begin{subtable}[t]{3.2in}
    \small
	\centering
	\setlength{\tabcolsep}{1.2mm}
	\small
	\begin{tabular}{l|ccccc}
    Layers & GFLOPS/FPS & \#params & ${\rm ID_{F1}}$  & ${\rm MOTA}$ & ${\rm MOTP}$  \\
    \hline
    % 2 & 59.2 & 42.1 & 76.2 & 36.7 & 30.2 \\
    3 & 94/10.4 & 38M & 61.6 & 44.6 & 76.3 \\
    4 & 104/9.8 & 39M & 64.3 & 46.4 & 76.6 \\
    5 & 114/8.9 & 40M & 65.1 & 47.2 & 76.3 \\
    6 & 124/8.4 & 41M & \textbf{65.5} & \textbf{47.5} & \textbf{76.2} \\
    
    
    % \whline
    \end{tabular}
    \caption{Effect of encoder size for text tracking task on ICDAR2015~(video)~\cite{karatzas2015icdar}.}
	\label{table:encoder}
	\vspace{2mm}
\end{subtable}
